Fairness and Consensus in an Asynchronous Opinion Model for Social Networks (Technical Report)

We introduce a DeGroot-based model for opinion dynamics in social networks. A community of agents is represented as a weighted directed graph whose edges indicate how much agents influence one another. The model is formalized using labeled transition systems, henceforth called opinion transition systems (OTS), whose states represent the agents' opinions and whose actions are the edges of the influence graph. If a transition labeled $(i,j)$ is performed, agent $j$ updates their opinion taking into account the opinion of agent $i$ and the influence $i$ has over $j$. We study (convergence to) opinion consensus among the agents of strongly-connected graphs with influence values in the interval $(0,1)$. We show that consensus cannot be guaranteed under the standard strong fairness assumption on transition systems. We derive that consensus is guaranteed under a stronger notion from the literature of concurrent systems; bounded fairness. We argue that bounded-fairness is too strong of a notion for consensus as it almost surely rules out random runs and it is not a constructive liveness property. We introduce a weaker fairness notion, called $m$-bounded fairness, and show that it guarantees consensus. The new notion includes almost surely all random runs and it is a constructive liveness property. Finally, we consider OTS with dynamic influence and show convergence to consensus holds under $m$-bounded fairness if the influence changes within a fixed interval $[L,U]$ with $0<L<U<1$. We illustrate OTS with examples and simulations, offering insights into opinion formation under fairness and dynamic influence.

==> figures/mCBFCounterexample_wrap.tex <==
\begin{wrapfigure}[21]{t}{0.5\textwidth}
\centering%
\begin{subfigure}[t]{0.5\textwidth}%
\centering%
    \begin{tikzpicture}[->, shorten >=1pt,node distance=1.5cm,semithick,
    inner sep=2pt,bend angle=45, initial text=,]
      \node[state, fill=green!70!gray] (1) {1};
      \node[state, fill=yellow!70!gray] (2) [right of=1] {2};
    \node[state, fill=red!50!gray] (3) [right of=2] {3};
      \node[state, fill=cyan!70!gray] (4) [right of=3] {4};
    
    \path(1) edge[right, anchor=south,  bend left=10] node{$a$}
    (2);

    \path(2) edge[left, anchor=north,  bend left=10] node{$b$}
    (1);

    \path(2) edge[right, anchor=south,  bend left=10] node{$d$}
    (3);

    \path(3) edge[left, anchor=north,  bend left=10] node{$c$}
    (2);

    \path(3) edge[right, anchor=south,  bend left=10] node{$f$}
    (4);
    
    \path(4) edge[left, anchor=north,  bend left=10] node{$e$}
    (3);



    \end{tikzpicture}

\caption{\label{fig:mCBFCounterexNetwork} Influence graph with $I_e = 1/2$ for all $e\in E$ and $\binit=(0.0,0.2,0.8,1.0)$.}
\end{subfigure}


\begin{subfigure}[t]{0.5\textwidth}%
\centering%
 \includegraphics[width=1.1\textwidth]{figures/pdf/mbfCounterex.pdf}
\caption{\label{fig:mCBFCounterexPlot} Opinion evolution of the $\omega$-word produced in \autoref{ex:mbfCounterEx} and $U=0.8$ and $L=0.2$. Each plot corresponds to the opinion of the agent with the same color in Fig. \ref{fig:mCBFCounterexNetwork}.}
\end{subfigure}

\caption{\label{fig:mCBFCounterex} Example of an $m$-bounded run for $m=1$ that does not converge to consensus.}

\end{wrapfigure}


==> figures/puppets.tex <==

\pgfplotstableread{figures/data_puppets.txt}
\datatable
\begin{wrapfigure}[15]{H}{0.4\textwidth}
\centering%
    \includegraphics[width=0.5\textwidth]{figures/pdf/puppetsCounterex.pdf}
\caption{\label{fig:puppets} Opinion evolution of the run $(abcd)^\omega$ for an OTS with $\graph$ and $\binit$ from \autoref{fig:ex1} but assuming $I_e=1$ for all $e \in \edges$. }
\end{wrapfigure}



==> sections/conclusion.tex <==
\section{Conclusion}
\label{sect:conclusions}
We have proposed a new formal model for interaction in opinion networks. It is based on the DeGroot model, but it allows for asynchronous interactions between agents. We have shown that our model might not converge to consensus under traditional fairness property assumptions. However, we also proved it can converge to consensus under certain conditions, including the ban of ``puppet'' agents. We also went over $k$-fairness, which can be found in the literature, but is not feasible, and proposed a new property called bounded wait, which is fulfilled by new notions like $k*$-fairness and $m$-consecutive bounded fairness. We have also shown that our model can be generalized to allow for dynamic influence between agents.

This work provides a foundation for further research on consensus in asynchronous gossip networks. We believe that novel mechanisms such as asynchrony and nondeterminism can capture new polarization and opinion dynamics. Our work provides a more realistic model of social network interactions, which can improve our understanding of models of interaction between intelligent agents. This work is part of the \href{https://sites.google.com/view/promueva/home}{PROMUEVA} project whose goal is to develop computational models and analysis techniques for social networks that incorporate elements such as communication, beliefs, and private and public messages. 

In the current work opinions are restricted to a given proposition and represented as a real value. Future work involves representing opinions as formulae from epistemic logic \cite{fagin1995reasoning} stating which each agent believes.  We plan to build upon our previous work on process calculi and epistemic models whose agent interact by exchanging beliefs (e.g., \cite{knight:hal-00761116,guzman:hal-02172415,haar:hal-01256984}). The problem of consensus in the resulting models could be expressed in terms convergence/reachability decision problems as the ones studied in \cite{palamidessi:inria-00201096,aranda:inria-00430531}
